Improving Neuroevolution Using Island Extinction and Repopulation

Neuroevolution commonly uses speciation strategies to better explore the search space of neural network architectures. One such speciation strategy is through the use of islands, which are also popular in improving performance and convergence of distributed evolutionary algorithms. However, in this approach some islands can become stagnant and not find new best solutions. In this paper, we propose utilizing extinction events and island repopulation to avoid premature convergence. We explore this with the Evolutionary eXploration of Augmenting Memory Models (EXAMM) neuro-evolution algorithm. In this strategy, all members of the worst performing island are killed of periodically and repopulated with mutated versions of the global best genome. This island based strategy is additionally compared to NEAT's (NeuroEvolution of Augmenting Topologies) speciation strategy. Experiments were performed using two different real world time series datasets (coal-fired power plant and aviation flight data). The results show that with statistical significance, this island extinction and repopulation strategy evolves better global best genomes than both EXAMM's original island based strategy and NEAT's speciation strategy.

==> 03-related_work.tex <==

Bio-inspired mata-heuristics are widely used to solve various optimization problems, as they are robust enough to solve complicated open-ended questions~\cite{binitha2012survey}~\cite{darwish2018bio}. ElSaid~\etal~evolved Long Short Term Memory (LSTM) cells in time series prediction with Ant Colony Optimization (ACO). Ants search through a large scale fully connected fixed topology for the best substructure network~\cite{elsaid2018optimizing}\cite{elsaid2018using}\cite{elsaid2016using}. And in Particle Swarm Optimization (PSO) algorithm, each particle evolves its own network by updating weights and topology~\cite{sahu2016evolving}\cite{wang2018evolving}\cite{yu2008evolving}. Conforth~\etal~showed ants and PSO can be combined to evolve ANNs in reinforcement learning~\cite{conforth2008toward}. Other bio-inspired algorithms such as Bird Swarm Algorithm (BSA)~\cite{aljarah2019evolving} and Artificial Bee Colony (ABC) ~\cite{zhu2019evolutionary} are also used to evolve ANNs.

One of the important aspects in EAs is speciation, which emphasizes to keep the diversity of the solutions. Groups of genomes develop into different directions to adapt to their niche. It provides more than one solutions to a problem. NEAT (Evolving Neural Networks through Augmenting Topologies)~\cite{stanley2002evolving}~ seperates genomes into different species by tracking historical genes and measuring the distance between the new genome and an existing species. By staring with a population of minimal genomes, NEAT finds solutions with fewer dimensions more efficiently. Another speciation algorithm Natural Evolution Speciation for NEAT (NENEAT)~\cite{knapp2019natural}~replaces NEAT's speciation strategy with cladistic, that all the genomes in the same species share a subset of nodes. So networks on a single path through a tree are same species. Hadjiivanov~\etal~designed a complexity-based speciation strategy, that is, grouping genomes by the number of hidden neurons~\cite{hadjiivanov2016complexity}. 

Other than strategies to divide genomes into different species, evolutionary rules such as mutation, crossover, weight initialization, and distance function, are also crucial to the speciation process. Verbancsics~\etal~investigated the effect of crossover and mutation on the NE speciation strategies. Sun~\etal~ applied a variable length gene encoding to avoid the network depth constrain for solving complex problems~\cite{sun2019evolving}. Krvcah~\etal~modified NEAT's fitness evaluation rule by changing the capacity of species dynamically~\cite{krvcah2012effects}. Instead of using objective functions to measure the fitness of a genome, Lehman~\etal~used searches for behavior novelty~\cite{lehman2011abandoning}. 

